Active Authentication on Mobile Devices via Stylometry, Application Usage, Web Browsing, and GPS Location

Active authentication is the problem of continuously verifying the identity of a person based on behavioral aspects of their interaction with a computing device. In this study, we collect and analyze behavioral biometrics data from 200subjects, each using their personal Android mobile device for a period of at least 30 days. This dataset is novel in the context of active authentication due to its size, duration, number of modalities, and absence of restrictions on tracked activity. The geographical colocation of the subjects in the study is representative of a large closed-world environment such as an organization where the unauthorized user of a device is likely to be an insider threat: coming from within the organization. We consider four biometric modalities: (1) text entered via soft keyboard, (2) applications used, (3) websites visited, and (4) physical location of the device as determined from GPS (when outdoors) or WiFi (when indoors). We implement and test a classifier for each modality and organize the classifiers as a parallel binary decision fusion architecture. We are able to characterize the performance of the system with respect to intruder detection time and to quantify the contribution of each modality to the overall performance.

==> images/stats-data/map-app-label-count.tex <==
\begin{table}[h]
  \centering
  \begin{tabular}{| l | l | }
    \hline
    TouchWiz home & 101,151\\\hline
    WhatsApp & 64,038\\\hline
    Messaging & 60,015\\\hline
    Launcher & 39,113\\\hline
    Facebook & 38,591\\\hline
    Google Search & 32,947\\\hline
    Chrome & 32,032\\\hline
    Snapchat & 23,481\\\hline
    System UI & 22,772\\\hline
    Phone & 19,396\\\hline
    Gmail & 19,329\\\hline
    Messages & 19,154\\\hline
    Contacts & 18,668\\\hline
    Hangouts & 17,209\\\hline
    Home & 16,775\\\hline
    HTC Sense & 16,325\\\hline
    com.google.android.youtube & 14,552\\\hline
    Xperia™ Home & 13,639\\\hline
    Instagram & 13,146\\\hline
    Settings & 12,675\\\hline
    Gallery & 11,832\\\hline
    TouchWiz Home & 11,691\\\hline
    Email & 10,908\\\hline
    Nova Launcher & 10,469\\\hline
    Clock & 9,186\\\hline
  \end{tabular}
\end{table}


==> images/stats-data/map-event-name-count.tex <==
\begin{table}[h]
  \centering
  \begin{tabular}{| l | l | }
    \hline
    Text & 23,254,478\\\hline
    App & 927,433\\\hline
    Web & 210,322\\\hline
    Location & 143,875\\\hline
  \end{tabular}
\end{table}


==> images/stats-data/map-event-name-rate.tex <==
\begin{table}[h]
  \centering
  \begin{tabular}{| l | l | }
    \hline
    Text & 557.811\\\hline
    App & 23.1865\\\hline
    Web & 5.56851\\\hline
    Location & 3.46248\\\hline
  \end{tabular}
\end{table}


==> images/stats-data/map-text-app-count.tex <==
\begin{table}[h]
  \centering
  \begin{tabular}{| l | l | }
    \hline
    com.android.sms & 5,617,297\\\hline
    com.android.mms & 5,552,079\\\hline
    com.whatsapp & 4,055,622\\\hline
    com.facebook.orca & 1,252,456\\\hline
    com.google.android.talk & 1,147,295\\\hline
    com.infraware.polarisviewer4 & 990,319\\\hline
    com.android.chrome & 417,165\\\hline
    com.facebook.katana & 405,267\\\hline
    com.snapchat.android & 377,840\\\hline
    com.google.android.gm & 271,570\\\hline
    com.htc.sense.mms & 238,300\\\hline
    com.tencent.mm & 221,461\\\hline
    com.motorola.messaging & 203,649\\\hline
    com.android.calculator2 & 167,435\\\hline
    com.verizon.messaging.vzmsgs & 137,339\\\hline
    com.groupme.android & 134,896\\\hline
    com.handcent.nextsms & 123,065\\\hline
    com.jb.gosms & 118,316\\\hline
    com.sonyericsson.conversations & 114,219\\\hline
    com.twitter.android & 92,605\\\hline
    com.google.android.googlequicksearchbox & 73,708\\\hline
    com.android.email & 63,545\\\hline
    com.tumblr & 57,778\\\hline
    com.tinder & 56,100\\\hline
    com.instagram.android & 54,411\\\hline
  \end{tabular}
\end{table}


==> images/stats-data/map-web-domain-count.tex <==
\begin{table}[h]
  \centering
  \begin{tabular}{| l | l | }
    \hline
    (search in url box) & 85,154\\\hline
    www.google.com & 19,004\\\hline
    m.facebook.com & 9,300\\\hline
    www.reddit.com & 4,348\\\hline
    forums.huaren.us & 3,093\\\hline
    learn.dcollege.net & 2,133\\\hline
    en.m.wikipedia.org & 1,825\\\hline
    mail.drexel.edu & 1,520\\\hline
    one.drexel.edu & 1,472\\\hline
    login.drexel.edu & 1,462\\\hline
    likes.com & 1,361\\\hline
    mail.google.com & 1,292\\\hline
    i.imgur.com & 1,132\\\hline
    www.amazon.com & 1,079\\\hline
    netcontrol.irt.drexel.edu & 1,049\\\hline
    www.facebook.com & 903\\\hline
    banner.drexel.edu & 902\\\hline
    m.hupu.com & 824\\\hline
    t.co & 801\\\hline
    duapp2.drexel.edu & 786\\\hline
    m.ign.com & 725\\\hline
    www.drexel.edu & 690\\\hline
    m.weibo.cn & 680\\\hline
    imgur.com & 651\\\hline
    muyuge.com & 599\\\hline
  \end{tabular}
\end{table}

